Cooperative Localization in WSNs: a Hybrid Convex/non-Convex Solution

We propose an efficient solution to peer-to-peer localization in a wireless sensor network which works in two stages. At the first stage the optimization problem is relaxed into a convex problem, given in the form recently proposed by Soares, Xavier, and Gomes. The convex problem is efficiently solved in a distributed way by an ADMM approach, which provides a significant improvement in speed with respect to the original solution. In the second stage, a soft transition to the original, non-convex, non relaxed formulation is applied in such a way to force the solution towards a local minimum. The algorithm is built in such a way to be fully distributed, and it is tested in meaningful situations, showing its effectiveness in localization accuracy and speed of convergence, as well as its inner robustness.

==> ALO4.tex <==
%\small
\SetKw{False}{False}		
\SetKw{True}{True}	

\For{iteration counter $t$ ranging from $0$ \KwTo $\infty$}{

\eIf{$t=0$}{
	Start from the convexified problem and set $F_i^\bullet = \tilde{F}_i$ as in \e{HY8}\\
	Initialize local positions $\B x_i=\B x_{i}^{0}$ \\	
	Initialize Lagrange multipliers $\B \lambda_{i}=\B 0$ \\
	Initialize penalty parameters $c_i=\epsilon_c$
}{	
	Update local positions $\B x_{i}$  via 
	$$
 \B x_{i}  \in \argmin_{\Bs x_i\in\C X_i} F_i^\bullet(\B x_i) + \fract12c_{i}(\B x_i -\B y_{i})^T\B D_i(\B x_i -\B y_{i})
 \e{AL16}
$$
with $\B y_{i} =\B D_i^{-1}\B A_i^T(\B z_{i}-\B\lambda_{i}/c_{i})$ and 
$$
\B D_i = \B A_i ^T \B A_i  = \qmatrix{
2 N_i \cr % &   \B 0_{N_i}^T\cr
 %\B 0_{N_i} 
 & 2 \B I_{N_i}
}\otimes\B I_n
\e{AL12}
$$
}

Build messages $\B m_{i}  = \B A_i\B x_{i}+ \B\lambda_{i}/c_{i}$

$\Rightarrow$ Broadcast values $c_i$, $\B m_{i,j}^+$, $\B m_{i,j}^-$ to  region $j\in\C N_i$

$\Leftarrow$ Receive values $c_j$, $\B m_{j,i}^+$, $\B m_{j,i}^-$  from  region $j\in\C N_i$

Extract the local projection on $\C Z$ by
$$
\eqalign{
\B z_{i,j}^{-} & = \fract12(\B m_{i,j}^- - \B m_{j,i}^-)\cr
\B z_{i,j}^{+} & = \fract12(\B m_{i,j}^+ + \B m_{j,i}^+)
}
\e{AL18}
$$

%\vspace*{-6mm}
\If{$t>0$}{
	Update Lagrange multipliers 
	$$
	\B \lambda_{i}=	\C P_{\lambda_{\max}}[\B \lambda_i+c_{i}\,(\B A_i\B x_{i}-\B z_{i})]
	\e{AL21}
	$$
	}
	
Evaluate the current primal gap
$$
\Gamma_{i} = \|\B A_i\B x_{i}-\B z_{i} \|_\infty
\e{AL22}
$$

\eIf{functionals are non-convex $F_i^\bullet = F_i$}{
Update penalty parameters
$$
c_{i} = \Big(\max_{j\in\C N_i\cup\{i\}}c_{j}\Big)  \cdot \cases{1&, $\Gamma_{i}\le\theta_c\Gamma_{i,\rm old}$\cr \delta_c &, otherwise}
\e{AL24}
$$
}{
\If{primal gap is sufficiently small $\Gamma_i<\tau_c$}{
	Activate the non-convex problem by setting $F_i^\bullet = F_i$ as in \e{HY4}\\
	Re-initialize penalty parameters $c_i=\zeta_c$
}
}

}

\caption{Cooperative algorithm at node $i$.}
\endinput




==> THY2.tex <==
\caption{Simulation settings}
\begin{center}
%\begin{small}
%\hspace*{-12mm}
\def\arraystretch{1.2}
\begin{tabular}{|c|c|c|c|}
\hline
& $N= 40$ & $N= 500$ & $N= 1000$ \\\hline
%SF & $?$ & $?$ & $?$ \\[2mm]\hline
\ac{ADMM}-SF & $\epsilon_c=0.005$ & $\epsilon_c=0.004$ & $\epsilon_c=0.002$ \\\hline
%\ac{SDP} & $?$ & $?$ & $?$ \\[2mm]\hline
\ac{ADMM}-NC & $\zeta_c=0.1$ & $\zeta_c=0.1$ & $\zeta_c=0.05$ \\\hline
\ac{ADMM}-H & $\epsilon_c=0.005$ & $\epsilon_c=0.004$ & $\epsilon_c=0.002$ \\
& $\zeta_c=0.1$ & $\zeta_c=0.2$ & $\zeta_c=0.05$ \\
& $\tau_c=0.04$ & $\tau_c=0.06$  & $\tau_c=0.02$  \\
\hline\end{tabular}
%\end{small}
\end{center}


